TaeBench: Improving Quality of Toxic Adversarial Examples

Toxicity text detectors can be vulnerable to adversarial examples - small perturbations to input text that fool the systems into wrong detection. Existing attack algorithms are time-consuming and often produce invalid or ambiguous adversarial examples, making them less useful for evaluating or improving real-world toxicity content moderators. This paper proposes an annotation pipeline for quality control of generated toxic adversarial examples (TAE). We design model-based automated annotation and human-based quality verification to assess the quality requirements of TAE. Successful TAE should fool a target toxicity model into making benign predictions, be grammatically reasonable, appear natural like human-generated text, and exhibit semantic toxicity. When applying these requirements to more than 20 state-of-the-art (SOTA) TAE attack recipes, we find many invalid samples from a total of 940k raw TAE attack generations. We then utilize the proposed pipeline to filter and curate a high-quality TAE dataset we call TaeBench (of size 264k). Empirically, we demonstrate that TaeBench can effectively transfer-attack SOTA toxicity content moderation models and services. Our experiments also show that TaeBench with adversarial training achieve significant improvements of the robustness of two toxicity detectors.

==> 00-preambular.tex <==


\usepackage{etoolbox}

\usepackage{graphicx}
\usepackage{float}
\usepackage[utf8]{inputenc}

\newcommand{\jennifer}[1]{\textcolor{blue}{#1 -[Jennifer]}}
\newcommand{\liwen}[1]{\textcolor{red}{#1 -[Liwen]}}
 
 \newcommand{\qnote}[1]{\textcolor{purple}{TODO:#1}}
\newcommand{\ninad}[1]{\textcolor{orange}{#1 -[Ninad]}}


\newcommand{\here}{\textcolor{purple}{\tt Q-edit ends here last time.}}




==> 07-more-bae.tex <==
\subsection{Running \bae Attacks} \label{sec:bae}
\tae examples are semantic-toxic samples that fool toxicity detectors to make benign (false negative) predictions.
Complementary to \tae, we search for semantic-benign samples that fool a target model into making toxic predictions.

To search for \bae, we design its goal function as: 
\begin{equation}
\label{eq:btae}
        \G(\F, \x') :=  \{ \F(\x') \neq b; \F(\x) = b \}
\end{equation}
where $b$ denotes the benign class. Starting from benign seeds ($\F(\x) = b$), we perturb $\x$ into $\x'$ by pushing the prediction of $\x'$ to not be benign anymore. We can reuse the \tae attack recipes by keeping their transformation, search and constraint components intact, and replace the goal function into the above \eref{eq:btae}.

Empirically, we run the 25 \bae attacks following the same setup as \bench, obtaining 102,667 raw \bae examples as a large unfiltered candidate pool. We automatically filter \bae examples using the proposed quality control pipeline, and combine filtered \bae to \tae to create a new benchmark dataset called \plus.


==> 07-more-recipe.tex <==
\subsection{TAE Attack Components} \label{sec:recipe}

\citet{morris2020reevaluating} propose splitting each text adversarial attack into four components: (1) goal function, (2) transformation, (3) search strategy, and (4) constraints between seed and its adversarial examples. This modular design allows pairing the \tae goal function (Eq-1) with popular choices of other three components from the literature to obtain a large set of \taee attack recipes.

\textbf{Transformation.} The attack recipes use different character or word transformation components. We also include the recipes using a combination of both character and word transformations.
Character transformation performs character insertion, deletion, neighboring swap, and replacements to change a word into one that a target toxicity detection model does not recognize.
Word transformation uses different methods including: synonym word replacement using WordNet; word substitution using BERT masked language model with 20 nearest neighbors; and word replacement using GLOVE word embedding with 5, 20, and 50 nearest neighbors.

\textbf{Constraints.} \taee recipes have differences in what language constraints they employ to limit the transformation. For instance, \atot puts limit on the number of words to perturb. \textbugger and {\tt ToxicTrap} use universal sentence encoding (USE) similarity as a constraint. We also include variants that optionally use Part-of-Speech constraints. These SOTA constraints aim to preserve semantics, grammar, and naturalness in creating attack examples.

\textbf{Search Method.} \taee attack recipes use greedy-based word importance ranking (Greedy-WIR) or beam search strategies to search and determine what words to transform, either by character perturbation or synonym replacement. When we use the Greedy-WIR strategy, we adopt different search methods based on gradient, deletion, unk masking, or weighted-saliency.


==> 07-table-tae.tex <==


\begin{table*}[htb]
    \centering
    \scalebox{0.95}{

    \begin{tabular}
    {p{2.4cm}|p{3.6cm}|p{5.3cm}|p{2.3cm}|p{1.3cm}}
    \hline
       
    \textbf{Attack Recipe} 
    & \textbf{Constraints} 
    & \textbf{Transformation}* 
    & \textbf{Search Method} & \textbf{\# of \tae Samples} \\ %
  \hline



     {\tt ToxicTrap} \newline from~\citep{bespalov-etal-2023-towards}: \newline
     20 recipe variants 
     
    & USE sentence encoding angular similarity $> 0.84$, with and without Part-of-Speech match, \newline Ratio of number of words modified $<0.1$
     & 
     Random Character Insertion, Random Character Deletion, Neighboring Character Swap, Character Substitution by Homoglyph$^\ddagger$, Word Synonym Replacement with $5$, $20$, or $50$ nearest      
     neighbors in the counter-fitted GLOVE word embedding space, or those predicted by BERT MLM model, or from WordNet. 
     
     & Greedy-WIR (gradient, delete, unk, or saliency-based), \newline genetic or beam search  & 623,548
     \\ \hline

  
     \atot \newline \newline (revised from \citep{a2t21})
    & Sentence-transformers/all-MiniLM-L6-v2 sentence encoding cosine similarity $> 0.9$$^\dagger$, Part-of-Speech match, Ratio of number of words modified $<0.1$ 
     & Word Synonym Replacement. Swap words with their 20 nearest neighbors in the counter-fitted GLOVE word embedding space or optionally with those predicted by BERT MLM model. 
     & Greedy-WIR (gradient-based)  & 36,634
     \\ \hline
     
    \textfooler \newline  \newline (revised from \citep{Jin2019TextFooler}  
    & Word embedding cosine similarity $>0.5$, Part-of-Speech match, USE sentence encoding angular similarity $ > 0.84$ 
     & Word Synonym Replacement. Swap words with their 50 nearest neighbors in the counter-fitted GLOVE word embedding space.  
     & Greedy-WIR (deletion-based) & 91,858
    \\\hline
    
    \pwws \newline \newline (revised from \citep{pwws-ren-etal-2019-generating}) 
     & No special constraints
     & Word Synonym Replacement. Swap words with synonyms from WordNet.  
     & Greedy-WIR (saliency) & 47,558

    
    \\\hline
    
    
     
     \deepbug \newline \newline (revised from \citep{Gao2018BlackBoxGO})
     
     & Levenshtein edit distance $< 30$
     & Random Character Insertion, Random Character Deletion, Random Character Swap, Random Character Replacement
     & Greedy-WIR (deletion-based) & 47,611
 
     \\ \hline

     \textbugger  \newline \newline (revised from \citep{Li2019TextBuggerGA})
    
     & USE sentence encoding cosine similarity $> 0.8$
     & Random Character Insertion, Random Character Deletion, Neighboring Character Swap, Character Substitution by Homoglyph$^\ddagger$, Word Synonym Replacement with 5 nearest neighbors in the counter-fitted GLOVE word embedding space
     &  Greedy-WIR (deletion-based) & 89,533
     \\ \hline
    
    \hline

    
    \end{tabular}
    
    
    }
    \caption{Attack recipes are categorized along: search method, transformations, and constraints. All attack recipes include an additional constraint which disallows replacing stopwords.
    \newline
\footnotesize{   \textit{$\dagger$ indicates new features or enhancements we added to extend the capability of the original attack recipes proposed in the original papers.}    
    \newline 
    \textit{* indicates a combination of multiple transformations}. 
    \hspace{3mm}
    \newline
    \textit{$\ddagger$ substitutes a character with visually similar ones or those adjacent on keyboard. For example, substitutes "1" with "l". }}
    }
    \label{table:categorized-attacks}
\end{table*}




 

Figure1: to point out a true challenge task 

Figure 2: schematic diagram 

Figure 3: performance 


Figure~\ref{fig:mot} shows one \tae adversarial example. The \tae replaces one word in the original text with its synonym to generate the perturbed text. The perturbed text and the original toxic text are semantically similar. Unfortunately, the perturbed text fooled the detector into a wrong detection (as "benign"). 


